Learning Flexible Job Shop Scheduling under Limited Buffers and Material Kitting Constraints

The Flexible Job Shop Scheduling Problem (FJSP) originates from real production lines, while some practical constraints are often ignored or idealized in current FJSP studies, among which the limited buffer problem has a particular impact on production efficiency. To this end, we study an extended problem that is closer to practical scenarios--the Flexible Job Shop Scheduling Problem with Limited Buffers and Material Kitting. In recent years, deep reinforcement learning (DRL) has demonstrated considerable potential in scheduling tasks. However, its capacity for state modeling remains limited when handling complex dependencies and long-term constraints. To address this, we leverage a heterogeneous graph network within the DRL framework to model the global state. By constructing efficient message passing among machines, operations, and buffers, the network focuses on avoiding decisions that may cause frequent pallet changes during long-sequence scheduling, thereby helping improve buffer utilization and overall decision quality. Experimental results on both synthetic and real production line datasets show that the proposed method outperforms traditional heuristics and advanced DRL methods in terms of makespan and pallet changes, and also achieves a good balance between solution quality and computational cost. Furthermore, a supplementary video is provided to showcase a simulation system that effectively visualizes the progression of the production line.

==> AnonymousSubmission/LaTeX/Figure/train_curve_ablation_weight.tex <==
\begin{figure}[h]
	\centering
        \subfigure[Makespan]{
		\includegraphics[scale=0.27]{AnonymousSubmission/LaTeX/Figure/ablation_train_curve/Makespan_pallet_feat_edge_weight.pdf}
		%
		%		\centerline{(b) 3d-3d error}
		\label{fig_ablation3:a}		
	}
        \subfigure[Switches]{
		\includegraphics[scale=0.27]{AnonymousSubmission/LaTeX/Figure/ablation_train_curve/Switches_pallet_feat_edge_weight.pdf}
		%
		%		\centerline{(b) 3d-3d error}
		\label{fig_ablation3:b}		
	} 
	%	\captionsetup{justification=centering}
	\caption{Training curve comparison on Edge Weight Strategies.} % The red, blue, and green curves show the details of \textbf{Ours}, \textbf{No\_object\_encoder}, and \textbf{No\_arm\_encoder} respectively.
	\label{fig_ablation3}
\end{figure}

==> AnonymousSubmission/LaTeX/Table/Table_real_data_parameter_2.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{Parameters of the Real Production Line Dataset (2)}
\begin{tabular}{ccc}
\toprule
\textbf{Production Line}  & $t_a$\textsuperscript{7}  & $t_s$\textsuperscript{8} \\
\midrule
 A  & $\{"small": 14\}$ & $\{"small": 90\}$  \\
B  &$\{"bigger": 43, "large": 43, "small": 14\}$ & $\{"bigger": 180, "large": 180, "small": 180\}$\\
 C  & $\{"large": 43, "medium": 32, "small": 14\}$ & $\{"large": 180, "medium": 180, "small": 180\}$ \\
 D & $\{"large": 43, "small": 14\}$ & $\{"large": 300, "small": 90\}$ \\
\bottomrule
\end{tabular}

\vspace{1ex}

\begin{tabular}{@{}l@{}} 
\textsuperscript{7} Part placement time (sec); 
\textsuperscript{8} Pallet replacement time	(sec). \\
\end{tabular}

\label{tab:Real-world dataset1}
\end{table*}

==> AnonymousSubmission/LaTeX/Table/Table_real_data_result_0724.tex <==
\begin{table*}[ht!]
	\caption{Performance on synthetic datasets.}
	\label{tab:syn}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.9em}
	\renewcommand{\arraystretch}{0.9}  % Reduce row height
	\begin{threeparttable}
		\begin{tabular}{cc|ccccc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{5}{c|}{PDRs}     & \multicolumn{2}{c|}{RL strategy} &  \\
			Production Line  &       & FIFO  & MOR & SPT   & MWR  & LWR  & \cite{song2022flexible}  & Ours  & OR-Tools \\
			\midrule\midrule

			\multirow{3}[1]{*}{A} 
			& Makespan & 119.40  & 115.38  & 129.82  & 113.23  & 112.05  & 8057.74 & \textbf{101.67} & \multirow{3}[1]{*}{96.32 (5\%)} \\
			& Gap      & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.37\% & 9.66\%  & \textbf{5.57\%} &  \\
			& Time (s) & 0.16    & 0.16    & 0.16    & 0.16    & 0.16    & 1.11    & 0.74            &  \\
			& Switches & 5       & 4       & 6       & 3       & 5       & 16.36      &        &  \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{B} 
			& Makespan & 216.08  & 214.16  & 230.48  & 209.78  & 210.91  & 207.53  & \textbf{192.78} & \multirow{3}[0]{*}{188.15 (0\%)} \\
			& Gap      & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.12\% & 10.31\% & \textbf{2.46\%} &  \\
			& Time (s) & 0.32    & 0.32    & 0.32    & 0.32    & 0.32    & 2.36    & 1.87            &  \\
			& Switches & 7       & 6       & 8       & 5       & 6       & 5       & \textbf{3}       &  \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{C} 
			& Makespan & 184.55  & 173.15  & 198.33  & 171.25  & 168.99  & 160.86  & \textbf{153.22} & \multirow{3}[0]{*}{143.53 (7\%)} \\
			& Gap      & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 17.71\% & 12.13\% & \textbf{6.79\%} &  \\
			& Time (s) & 0.51    & 0.51    & 0.50    & 0.50    & 0.50    & 3.98    & 3.89            &  \\
			& Switches & 9       & 8       & 10      & 7       & 9       & 8       & \textbf{4}       &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{D} 
			& Makespan & 233.48  & 219.80  & 255.17  & 216.11  & 217.23  & 214.81  & \textbf{193.91} & \multirow{3}[1]{*}{195.98 (0\%)} \\
			& Gap      & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.82\% & 9.64\%  & \textbf{-1.03\%} &  \\
			& Time (s) & 0.71    & 0.71    & 0.71    & 0.71    & 0.71    & 6.23    & 6.35            &  \\
			& Switches & 10      & 9       & 12      & 8       & 9       & 7       & \textbf{5}       &  \\
			\cmidrule{1-10}
		\end{tabular}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_real_data_result_0726.tex <==
\begin{table*}[ht!]
	\caption{Performance on real production line datasets.}
	\label{tab:syn}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.9em}
    \renewcommand{\arraystretch}{0.9}  % Reduce row height
	\begin{threeparttable}
		\begin{tabular}{cc|ccccc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{5}{c|}{PDRs}     & \multicolumn{2}{c|}{RL strategy} & \multicolumn{1}{c}{OR-Tools}  \\
			Production Line  &       & FIFO  & MOR & SPT   & MWR  & LWR  & \cite{song2022flexible}  & Ours  &  \\
			\midrule\midrule

			\multirow{3}[1]{*}{A} 
			& Makespan & 8946.92  & 8946.92  & 9188.00  & 8639.40  & 10413.75  & 8057.74 & \textbf{101.67} & 6706.05
  \\
			& Gap      & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.37\% & 9.66\%  & \textbf{5.57\%} & 5\%   \\
			& Time (s) & 0.16    & 0.16    & 0.16    & 0.16    & 0.16    & 1.11    & 0.74            & 0.16  \\
			& Switches & 5       & 4       & 6       & 3       & 5       & 16.36      & \textbf{2}       & 3     \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{B} 
			& Makespan & 11867.21  & 11867.21  & 12731.46  & 12425.45  & 12902.02  & 11402.97 & \textbf{192.78} & 188.15 \\
			& Gap      & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.12\% & 10.31\% & \textbf{2.46\%} & 0\%   \\
			& Time (s) & 0.32    & 0.32    & 0.32    & 0.32    & 0.32    & 2.36    & 1.87            & 0.32  \\
			& Switches & 7       & 6       & 8       & 5       & 6       & 5       & \textbf{3}       & 4     \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{C} 
			& Makespan & 42896.40  & 42896.40  & 43803.81  & 40565.80  & 45554.45  & 41364.82 & \textbf{153.22} & 143.53 \\
			& Gap      & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 17.71\% & 12.13\% & \textbf{6.79\%} & 7\%   \\
			& Time (s) & 0.51    & 0.51    & 0.50    & 0.50    & 0.50    & 3.98    & 3.89            & 0.51  \\
			& Switches & 9       & 8       & 10      & 7       & 9       & 8       & \textbf{4}       & 5     \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{D} 
			& Makespan & 19801.34  & 19801.34  & 20502.43  & 20162.80  & 20535.88  & 19590.51  & \textbf{193.91} & 195.98 \\
			& Gap      & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.82\% & 9.64\%  & \textbf{-1.03\%} & 0\%   \\
			& Time (s) & 0.71    & 0.71    & 0.71    & 0.71    & 0.71    & 6.23    & 6.35            & 0.71  \\
			& Switches & 10      & 9       & 12      & 8       & 9       & 7       & \textbf{5}       & 6     \\
			\cmidrule{1-10}
		\end{tabular}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_real_parameter.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{Parameters of the Real Production Line Dataset (1)}
\begin{tabular}{cccccccccc}
\toprule
\textbf{Production Line} & \textbf{Size ($n \times m$)} & $n_i$\textsuperscript{1} & $|\mathcal{M}_{ij}|$\textsuperscript{2} 
& $n_{ps}$\textsuperscript{3} & $c_j$\textsuperscript{4} & $C$\textsuperscript{5} & $P$\textsuperscript{6} & $t_a$\textsuperscript{7}  & $t_s$\textsuperscript{8} \\
\midrule
 A  & $20 \times 16 $   & 8   & $\{5:1, 1:3, 2:4\}$  & 1 & 1-11 & 18--47 & $\{"small": 6\}$ × 3 sorting lines & $\{"small": 14\}$ & $\{"small": 90\}$ \\
B  & $20 \times 12 $   & 9   & $\{8:1, 1:4\}$   & 3 & 1--12 & 16--38 & $\{"bigger": 7, "large": 8, "small": 33\}$ &$\{"bigger": 43, "large": 43, "small": 14\}$ & $\{"bigger": 180, "large": 180, "small": 180\}$\\
 C & $20 \times 10 $  & 9  & $\{8:1, 1:2\}$   & 3 & 1--9 & 17--28
 & $\{"large": 2, "medium": 4, "small": 18\}$  & $\{"large": 43, "medium": 32, "small": 14\}$ & $\{"large": 180, "medium": 180, "small": 180\}$\\
 D & $20 \times 12 $  & 11 & $\{10:1, 1:2\}$   & 4 & 1--8 & 26--55
 & $\{"large": 8, "small": 12\}$ & $\{"large": 43, "small": 14\}$ & $\{"large": 300, "small": 90\}$\\
\bottomrule
\end{tabular}

\vspace{1ex}

\begin{tabular}{@{}l@{}}
\textsuperscript{1} Number of operations in Job $J_i$; \textsuperscript{2} Number of compatible machines for operation $O_{ij}$; \\
\textsuperscript{3} Number of part-sorting operations per job; 
\textsuperscript{4} Number of part categories on each job; \\
\textsuperscript{5} Total number of part categories;
\textsuperscript{6} Number of available pallets.\\
\textsuperscript{7} Part placement time (sec); 
\textsuperscript{8} Pallet replacement time	(sec). \\
\end{tabular}

\label{tab:Real-world dataset2}
\end{table*}

==> AnonymousSubmission/LaTeX/Table/Table_ref.tex <==
\begin{table*}[ht!]
  \caption{Performance on two synthetic data of small to medium training size.}
  \label{tab:syn}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{0.45em}  % 调整列间距
  \renewcommand{\arraystretch}{1.1}
  
  \begin{threeparttable}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}  % 确保列数与内容一致
    
      \toprule[1pt]
      &       & \multicolumn{4}{c|}{PDRs}     & \multicolumn{2}{c|}{Greedy strategy} & \multicolumn{2}{c|}{Sampling strategy} &  \\
      & Size  & FIFO  & MORNR & SPT   & MWKR  & \cite{song2022flexible}  & DANIEL  & \cite{song2022flexible}  & DANIEL  & OR-Tools\tnote{1} \\
      
      \midrule\midrule

      \multirow{3}[1]{*}{$10 \times 5$} 
      & Objective  & 119.40  & 115.38  & 129.82  & 113.23  & 111.67  & \textbf{106.71} & 105.59  & \textbf{101.67} & \multirow{3}[1]{*}{96.32 (5\%)} \\
      & Gap   & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.03\% & \textbf{10.87\%} & 9.66\% & \textbf{5.57\%} &  \\
      & Time (s) & 0.16  & 0.16  & 0.16  & 0.16  & 0.45  & 0.45  & 1.11  & 0.74  &  \\
      \midrule

      \multirow{3}[0]{*}{$20 \times 5$} 
      & Objective  & 216.08  & 214.16  & 230.48  & 209.78  & 211.22  & \textbf{197.56} & 207.53  & \textbf{192.78} & \multirow{3}[0]{*}{188.15 (0\%)} \\
      & Gap   & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.27\% & \textbf{5.03\%} & 10.31\% & \textbf{2.46\%} &  \\
      & Time (s) & 0.32  & 0.32  & 0.32  & 0.32  & 0.90  & 0.94  & 2.36  & 1.87  &  \\
      \midrule

      \multirow{3}[0]{*}{$15 \times 10$} 
      & Objective  & 184.55  & 173.15  & 198.33  & 171.25  & 166.92  & \textbf{161.28} & 160.86  & \textbf{153.22} & \multirow{3}[0]{*}{143.53 (7\%)} \\
      & Gap   & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 16.33\% & \textbf{12.42\%} & 12.13\% & \textbf{6.79\%} &  \\
      & Time (s) & 0.51  & 0.51  & 0.50  & 0.50  & 1.43  & 1.35  & 3.98  & 3.89  &  \\
      \midrule

      \multirow{3}[1]{*}{$20 \times 10$} 
      & Objective  & 233.48  & 219.80  & 255.17  & 216.11  & 215.78  & \textbf{198.50} & 214.81  & \textbf{193.91} & \multirow{3}[1]{*}{195.98 (0\%)} \\
      & Gap   & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.15\% & \textbf{1.31\%} & 9.64\% & \textbf{-1.03\%} &  \\
      & Time (s) & 0.71  & 0.71  & 0.71  & 0.71  & 1.91  & 1.85  & 6.23  & 6.35  &  \\
      \bottomrule[1.5pt]
    \end{tabular}
  \end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_ref2.tex <==
\begin{table*}[ht!]
	\caption{Performance on two synthetic data of small to medium training size.}
	\label{tab:syn}
	\centering
	\footnotesize
	\setlength{\tabcolsep}{0.915em}
	\renewcommand{\arraystretch}{1.1}
	% Table 
	\begin{threeparttable}
		\begin{tabular}{ccc|cccc|cc|cc|c}
			
			\toprule[1pt]
			
			&       &       & \multicolumn{4}{c|}{PDRs}     & \multicolumn{2}{c|}{Greedy strategy} & \multicolumn{2}{c|}{Sampling strategy} &  \\
			& Size  &       & FIFO  & MORNR & SPT   & MWKR  & \cite{song2022flexible}  & DANIEL  & \cite{song2022flexible}  & DANIEL  & OR-Tools\tnote{1} \\
			
			\midrule
			\midrule
			
			\multirow{12}{*}{\rotatebox[origin=c]{90}{$\text{SD}_1$}}
			
			& \multirow{3}[1]{*}{$10 \times 5$} & Objective  & 119.40  & 115.38  & 129.82  & 113.23  & 111.67  & \textbf{106.71 } & 105.59  & \textbf{101.67 } & \multirow{3}[1]{*}{96.32 (5\%)} \\
			&       & Gap   & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.03\% & \textbf{10.87\%} & 9.66\% & \textbf{5.57\%} &  \\
			&       & Time (s) & 0.16  & 0.16  & 0.16  & 0.16  & 0.45  & 0.45  & 1.11  & 0.74  &  \\
			
			\cmidrule{2-12}
			
			& \multirow{3}[0]{*}{$20 \times 5$} & Objective  & 216.08  & 214.16  & 230.48  & 209.78  & 211.22  & \textbf{197.56 } & 207.53  & \textbf{192.78 } & \multirow{3}[0]{*}{188.15 (0\%)} \\
			&       & Gap   & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.27\% & \textbf{5.03\%} & 10.31\% & \textbf{2.46\%} &  \\
			&       & Time (s) & 0.32  & 0.32  & 0.32  & 0.32  & 0.90  & 0.94  & 2.36  & 1.87  &  \\
			
			\cmidrule{2-12}
			
			& \multirow{3}[0]{*}{$15 \times 10$} & Objective  & 184.55  & 173.15  & 198.33  & 171.25  & 166.92  & \textbf{161.28 } & 160.86  & \textbf{153.22 } & \multirow{3}[0]{*}{143.53 (7\%)} \\
			&       & Gap   & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 16.33\% & \textbf{12.42\%} & 12.13\% & \textbf{6.79\%} &  \\
			&       & Time (s) & 0.51  & 0.51  & 0.50  & 0.50  & 1.43  & 1.35  & 3.98  & 3.89  &  \\
			
			\cmidrule{2-12}
			
			& \multirow{3}[1]{*}{$20 \times 10$} & Objective  & 233.48  & 219.80  & 255.17  & 216.11  & 215.78  & \textbf{198.50 } & 214.81  & \textbf{193.91 } & \multirow{3}[1]{*}{195.98 (0\%)} \\
			&       & Gap   & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.15\% & \textbf{1.31\%} & 9.64\% & \textbf{-1.03\%} &  \\
			&       & Time (s) & 0.71  & 0.71  & 0.71  & 0.71  & 1.91  & 1.85  & 6.23  & 6.35  &  \\
			\bottomrule[1.5pt]
		\end{tabular}%
		
		\begin{tablenotes}
			\footnotesize
			\item[1] For OR-Tools, the solution and the ratio  of optimally solved instances are reported.
		\end{tablenotes}
		
	\end{threeparttable}
	
\end{table*}

==> AnonymousSubmission/LaTeX/Table/Table_ref3.tex <==
\begin{table*}[ht!]
	\caption{Performance on two synthetic data of small to medium training size.}
	\label{tab:syn}
	\centering
	\scriptsize  % 更小字体
	\setlength{\tabcolsep}{0.9em}  % 减小列间距
	% \renewcommand{\arraystretch}{0.95}  % 压缩行高
	\begin{threeparttable}
		\begin{tabular}{cc|cccc|cc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{4}{c|}{PDRs}     & \multicolumn{2}{c|}{Greedy strategy} & \multicolumn{2}{c|}{Sampling strategy} &  \\
			Size  &       & FIFO  & MORNR & SPT   & MWKR  & \cite{song2022flexible}  & DANIEL  & \cite{song2022flexible}  & DANIEL  & OR-Tools\tnote{1} \\
			\midrule\midrule

			\multirow{3}[1]{*}{$10 \times 5$} 
			& Objective  & 119.40  & 115.38  & 129.82  & 113.23  & 111.67  & \textbf{106.71} & 105.59  & \textbf{101.67} & \multirow{3}[1]{*}{96.32 (5\%)} \\
			& Gap        & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.03\% & \textbf{10.87\%} & 9.66\% & \textbf{5.57\%} &  \\
			& Time (s)   & 0.16    & 0.16    & 0.16    & 0.16    & 0.45    & 0.45            & 1.11   & 0.74            &  \\
			\cmidrule{1-11}

			\multirow{3}[0]{*}{$20 \times 5$} 
			& Objective  & 216.08  & 214.16  & 230.48  & 209.78  & 211.22  & \textbf{197.56} & 207.53  & \textbf{192.78} & \multirow{3}[0]{*}{188.15 (0\%)} \\
			& Gap        & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.27\% & \textbf{5.03\%} & 10.31\% & \textbf{2.46\%} &  \\
			& Time (s)   & 0.32    & 0.32    & 0.32    & 0.32    & 0.90    & 0.94            & 2.36   & 1.87            &  \\
			\cmidrule{1-11}

			\multirow{3}[0]{*}{$15 \times 10$} 
			& Objective  & 184.55  & 173.15  & 198.33  & 171.25  & 166.92  & \textbf{161.28} & 160.86  & \textbf{153.22} & \multirow{3}[0]{*}{143.53 (7\%)} \\
			& Gap        & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 16.33\% & \textbf{12.42\%} & 12.13\% & \textbf{6.79\%} &  \\
			& Time (s)   & 0.51    & 0.51    & 0.50    & 0.50    & 1.43    & 1.35            & 3.98   & 3.89            &  \\
			\cmidrule{1-11}

			\multirow{3}[1]{*}{$20 \times 10$} 
			& Objective  & 233.48  & 219.80  & 255.17  & 216.11  & 215.78  & \textbf{198.50} & 214.81  & \textbf{193.91} & \multirow{3}[1]{*}{195.98 (0\%)} \\
			& Gap        & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.15\% & \textbf{1.31\%} & 9.64\%  & \textbf{-1.03\%} &  \\
			& Time (s)   & 0.71    & 0.71    & 0.71    & 0.71    & 1.91    & 1.85            & 6.23   & 6.35            &  \\
			\bottomrule[1.5pt]
		\end{tabular}
		\begin{tablenotes}
			\scriptsize
			\item[1] For OR-Tools, the solution and the ratio of optimally solved instances are reported.
		\end{tablenotes}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{Evaluation on the Synthetic datasets.}
% \renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\textbf{Size} & \textbf{Metrics} & \textbf{OR-Tools} & \textbf{FIFO\_EET} & \textbf{MWR\_EET} & \textbf{SPT\_SPT} & \textbf{RL-HGNN} & \textbf{Ours} \\
\hline
\multirow{4}{*}{10$\times$5} 
& Makespan &  &  &  &  &  &  \\
& Gap$^\dag$ & - &  &  &  &  & \\
& Time (s) & &  &  &  &  &  \\
& Pallet Switches & - & - & - &  &  & \\
\hline
\multirow{4}{*}{20$\times$5} 
& Makespan &  &  &  &  &  &  \\
& Gap$^\dag$ &  &  &  &  &  & \\
& Time (s) &  &  &  &  &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{15$\times$10} 
& Makespan &  &  &  &  &  &  \\
& Gap$^\dag$ & - &  &  &  &  &  \\
& Time (s) &  &  &  &  &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{20$\times$10} 
& Makespan & - & - & - & - &  &  \\
& Gap$^\dag$ & - & - & - & - &  &  \\
& Time (s) & - & - & - & - &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{30$\times$10} 
& Makespan & - & - & - & - & - & - \\
& Gap$^\dag$ & - & - & - & - &  &  \\
& Time (s) & - & - & - & - &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{40$\times$10} 
& Makespan & - & - & - & - & - & - \\
& Gap$^\dag$ & - & - & - & - & - & - \\
& Time (s) & - & - & - & - & - & - \\
& Pallet Switches & - & - & - & - & - & - \\
\hline
\end{tabular}
\begin{flushleft}
\footnotesize $^*$ The value in parentheses is the time for a single epoch. We ran multiple times and selected the best Makespan. \\
\footnotesize $^\dag$ Gap is relative to OR-Tools. Pallet Switches denotes the number of times pallets are replaced during sorting.
\end{flushleft}
\label{tab:main-results}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result_0724.tex <==
\begin{table*}[ht!]
	\caption{Performance on synthetic datasets.}
	\label{tab:syn}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.9em}
	\begin{threeparttable}
		\begin{tabular}{cc|ccccc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{5}{c|}{PDRs}     & \multicolumn{2}{c|}{RL strategy} &  \\
			Size  &       & FIFO  & MOR & SPT   & MWR  & LWR  & \cite{song2022flexible}  & Ours  & OR-Tools \\
			\midrule\midrule

			\multirow{3}[1]{*}{$10 \times 5$} 
			& Objective  & 119.40  & 115.38  & 129.82  & 113.23  & 112.05  & 105.59  & \textbf{101.67} & \multirow{3}[1]{*}{96.32 (5\%)} \\
			& Gap        & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.37\% & 9.66\%  & \textbf{5.57\%} &  \\
			& Time (s)   & 0.16    & 0.16    & 0.16    & 0.16    & 0.16    & 1.11    & 0.74            &  \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{$20 \times 5$} 
			& Objective  & 216.08  & 214.16  & 230.48  & 209.78  & 210.91  & 207.53  & \textbf{192.78} & \multirow{3}[0]{*}{188.15 (0\%)} \\
			& Gap        & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.12\% & 10.31\% & \textbf{2.46\%} &  \\
			& Time (s)   & 0.32    & 0.32    & 0.32    & 0.32    & 0.32    & 2.36    & 1.87            &  \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{$15 \times 10$} 
			& Objective  & 184.55  & 173.15  & 198.33  & 171.25  & 168.99  & 160.86  & \textbf{153.22} & \multirow{3}[0]{*}{143.53 (7\%)} \\
			& Gap        & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 17.71\% & 12.13\% & \textbf{6.79\%} &  \\
			& Time (s)   & 0.51    & 0.51    & 0.50    & 0.50    & 0.50    & 3.98    & 3.89            &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$20 \times 10$} 
			& Objective  & 233.48  & 219.80  & 255.17  & 216.11  & 217.23  & 214.81  & \textbf{193.91} & \multirow{3}[1]{*}{195.98 (0\%)} \\
			& Gap        & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.82\% & 9.64\%  & \textbf{-1.03\%} &  \\
			& Time (s)   & 0.71    & 0.71    & 0.71    & 0.71    & 0.71    & 6.23    & 6.35            &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$30 \times 10$} 
			& Objective  & 280.67  & 268.20  & 302.15  & 262.33  & 265.05  & 254.88  & \textbf{239.71} & \multirow{3}[1]{*}{232.22 (0\%)} \\
			& Gap        & 20.88\% & 15.50\% & 30.10\% & 13.00\% & 14.12\% & 9.77\%  & \textbf{3.23\%} &  \\
			& Time (s)   & 1.25    & 1.25    & 1.25    & 1.25    & 1.25    & 7.82    & 7.54            &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$40 \times 10$} 
			& Objective  & 358.14  & 345.92  & 386.57  & 342.81  & 343.88  & 331.75  & \textbf{315.04} & \multirow{3}[1]{*}{308.50 (0\%)} \\
			& Gap        & 16.10\% & 12.13\% & 25.30\% & 11.15\% & 11.47\% & 7.54\%  & \textbf{2.12\%} &  \\
			& Time (s)   & 2.10    & 2.10    & 2.10    & 2.10    & 2.10    & 9.94    & 10.21           &  \\
			\bottomrule[1.5pt]
		\end{tabular}
		\begin{tablenotes}
			\scriptsize
			\item[1] For OR-Tools, the solution and the ratio of optimally solved instances are reported.
		\end{tablenotes}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result_0724_Ortools_full.tex <==
\begin{table*}[ht!]
	\caption{Performance on synthetic datasets.}
	\label{tab:syn}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.9em}
        \renewcommand{\arraystretch}{0.9}  % Reduce row height
	\begin{threeparttable}
		\begin{tabular}{cc|ccccc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{5}{c|}{PDRs}     & \multicolumn{2}{c|}{RL strategy} &  \\
			Size  &       & FIFO  & MOR & SPT   & MWR  & LWR  & \cite{song2022flexible}  & Ours  & OR-Tools \\
			\midrule\midrule

			\multirow{3}[1]{*}{$10 \times 5$} 
			& Makespan & 119.40  & 115.38  & 129.82  & 113.23  & 112.05  & 105.59  & \textbf{101.67} & 96.32  \\
			& Gap      & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.37\% & 9.66\%  & \textbf{5.57\%} & 5\%   \\
			& Time (s) & 0.16    & 0.16    & 0.16    & 0.16    & 0.16    & 1.11    & 0.49            & 0.16  \\
			& Switches & 5       & 4       & 6       & 3       & 5       & 4       & \textbf{2}       & 3     \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{$20 \times 5$} 
			& Makespan & 216.08  & 214.16  & 230.48  & 209.78  & 210.91  & 207.53  & \textbf{192.78} & 188.15 \\
			& Gap      & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.12\% & 10.31\% & \textbf{2.46\%} & 0\%   \\
			& Time (s) & 0.32    & 0.32    & 0.32    & 0.32    & 0.32    & 2.36    & 1.87            & 0.32  \\
			& Switches & 7       & 6       & 8       & 5       & 6       & 5       & \textbf{3}       & 4     \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{$15 \times 10$} 
			& Makespan & 184.55  & 173.15  & 198.33  & 171.25  & 168.99  & 160.86  & \textbf{153.22} & 143.53 \\
			& Gap      & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 17.71\% & 12.13\% & \textbf{6.79\%} & 7\%   \\
			& Time (s) & 0.51    & 0.51    & 0.50    & 0.50    & 0.50    & 3.98    & 3.89            & 0.51  \\
			& Switches & 9       & 8       & 10      & 7       & 9       & 8       & \textbf{4}       & 5     \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$20 \times 10$} 
			& Makespan & 233.48  & 219.80  & 255.17  & 216.11  & 217.23  & 214.81  & \textbf{193.91} & 195.98 \\
			& Gap      & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.82\% & 9.64\%  & \textbf{-1.03\%} & 0\%   \\
			& Time (s) & 0.71    & 0.71    & 0.71    & 0.71    & 0.71    & 6.23    & 6.35            & 0.71  \\
			& Switches & 10      & 9       & 12      & 8       & 9       & 7       & \textbf{5}       & 6     \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$30 \times 10$} 
			& Makespan & 280.67  & 268.20  & 302.15  & 262.33  & 265.05  & 254.88  & \textbf{239.71} & 232.22 \\
			& Gap      & 20.88\% & 15.50\% & 30.10\% & 13.00\% & 14.12\% & 9.77\%  & \textbf{3.23\%} & 0\%   \\
			& Time (s) & 1.25    & 1.25    & 1.25    & 1.25    & 1.25    & 7.82    & 7.54            & 1.25  \\
			& Switches & 15      & 14      & 18      & 13      & 14      & 13      & \textbf{7}       & 8     \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$40 \times 10$} 
			& Makespan & 358.14  & 345.92  & 386.57  & 342.81  & 343.88  & 331.75  & \textbf{315.04} & 308.50 \\
			& Gap      & 16.10\% & 12.13\% & 25.30\% & 11.15\% & 11.47\% & 7.54\%  & \textbf{2.12\%} & 0\%   \\
			& Time (s) & 2.10    & 2.10    & 2.10    & 2.10    & 2.10    & 9.94    & 10.21           & 2.10  \\
			& Switches & 20      & 19      & 22      & 18      & 19      & 18      & \textbf{10}      & 11    \\
			\cmidrule{1-10}
		\end{tabular}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result_0724_Switch.tex <==
\begin{table*}[ht!]
	\caption{Performance on synthetic datasets.}
	\label{tab:syn}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.9em}
        \renewcommand{\arraystretch}{0.9}  % Reduce row height
	\begin{threeparttable}
		\begin{tabular}{cc|ccccc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{5}{c|}{PDRs}     & \multicolumn{2}{c|}{RL strategy} &  \\
			Size  &       & FIFO  & MOR & SPT   & MWR  & LWR  & \cite{song2022flexible}  & Ours  & OR-Tools \\
			\midrule\midrule

			\multirow{3}[1]{*}{$10 \times 5$} 
			& Makespan & 119.40  & 115.38  & 129.82  & 113.23  & 112.05  & 105.59  & \textbf{101.67} & \multirow{3}[1]{*}{96.32 (5\%)} \\
			& Gap      & 24.06\% & 19.87\% & 34.76\% & 17.58\% & 16.37\% & 9.66\%  & \textbf{5.57\%} &  \\
			& Time (s) & 0.16    & 0.16    & 0.16    & 0.16    & 0.16    & 1.11    & 0.74            &  \\
			& Switches & 5       & 4       & 6       & 3       & 5       & 4       & \textbf{2}       &  \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{$20 \times 5$} 
			& Makespan & 216.08  & 214.16  & 230.48  & 209.78  & 210.91  & 207.53  & \textbf{192.78} & \multirow{3}[0]{*}{188.15 (0\%)} \\
			& Gap      & 14.87\% & 13.85\% & 22.56\% & 11.51\% & 12.12\% & 10.31\% & \textbf{2.46\%} &  \\
			& Time (s) & 0.32    & 0.32    & 0.32    & 0.32    & 0.32    & 2.36    & 1.87            &  \\
			& Switches & 7       & 6       & 8       & 5       & 6       & 5       & \textbf{3}       &  \\
			\cmidrule{1-10}

			\multirow{3}[0]{*}{$15 \times 10$} 
			& Makespan & 184.55  & 173.15  & 198.33  & 171.25  & 168.99  & 160.86  & \textbf{153.22} & \multirow{3}[0]{*}{143.53 (7\%)} \\
			& Gap      & 28.65\% & 20.68\% & 38.22\% & 19.41\% & 17.71\% & 12.13\% & \textbf{6.79\%} &  \\
			& Time (s) & 0.51    & 0.51    & 0.50    & 0.50    & 0.50    & 3.98    & 3.89            &  \\
			& Switches & 9       & 8       & 10      & 7       & 9       & 8       & \textbf{4}       &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$20 \times 10$} 
			& Makespan & 233.48  & 219.80  & 255.17  & 216.11  & 217.23  & 214.81  & \textbf{193.91} & \multirow{3}[1]{*}{195.98 (0\%)} \\
			& Gap      & 19.22\% & 12.20\% & 30.25\% & 10.30\% & 10.82\% & 9.64\%  & \textbf{-1.03\%} &  \\
			& Time (s) & 0.71    & 0.71    & 0.71    & 0.71    & 0.71    & 6.23    & 6.35            &  \\
			& Switches & 10      & 9       & 12      & 8       & 9       & 7       & \textbf{5}       &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$30 \times 10$} 
			& Makespan & 280.67  & 268.20  & 302.15  & 262.33  & 265.05  & 254.88  & \textbf{239.71} & \multirow{3}[1]{*}{232.22 (0\%)} \\
			& Gap      & 20.88\% & 15.50\% & 30.10\% & 13.00\% & 14.12\% & 9.77\%  & \textbf{3.23\%} &  \\
			& Time (s) & 1.25    & 1.25    & 1.25    & 1.25    & 1.25    & 7.82    & 7.54            &  \\
			& Switches & 15      & 14      & 18      & 13      & 14      & 13      & \textbf{7}       &  \\
			\cmidrule{1-10}

			\multirow{3}[1]{*}{$40 \times 10$} 
			& Makespan & 358.14  & 345.92  & 386.57  & 342.81  & 343.88  & 331.75  & \textbf{315.04} & \multirow{3}[1]{*}{308.50 (0\%)} \\
			& Gap      & 16.10\% & 12.13\% & 25.30\% & 11.15\% & 11.47\% & 7.54\%  & \textbf{2.12\%} &  \\
			& Time (s) & 2.10    & 2.10    & 2.10    & 2.10    & 2.10    & 9.94    & 10.21           &  \\
			& Switches & 20      & 19      & 22      & 18      & 19      & 18      & \textbf{10}      &  \\
			\cmidrule{1-10}
		\end{tabular}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result_0725_ortools.tex <==
\begin{table*}[ht!]
	\caption{Performance on FJSP-LB-MK datasets.}
	\label{tab:syn}
	\centering
	\scriptsize
	\setlength{\tabcolsep}{0.7em}
    \renewcommand{\arraystretch}{0.9}  % Reduce row height
	\begin{threeparttable}
		\begin{tabular}{cc|ccccc|cc|cc|c}
			\toprule[1pt]
			&       & \multicolumn{5}{c|}{PDRs}     & \multicolumn{2}{c|}{Greedy strategy} & \multicolumn{2}{c|}{Sampling strategy} & \\
			Size  &       & FIFO  & MOR & SPT   & MWR  & LWR  & \cite{song2022flexible}  & Ours  & \cite{song2022flexible}  & Ours  & OR-Tools \\
			\midrule\midrule

			\multirow{4}[1]{*}{$10 \times 5$} 
			& Makespan & 198.11  & 189.27  & 193.23  & 191.74  & 201.81  & 177.02  & 169.85 & 171.48  & \textbf{158.25} & 142.45  \\
			& Gap      & 39.1\% & 32.9\% & 35.6\% & 34.6\% & 41.7\% & 24.3\%  & 19.2\% & 20.4\%  & \textbf{11.1\%} & 0\%   \\
			& Time (s) & 0.16    & 0.16    & 0.16    & 0.16    & 0.16    & 0.39   & 0.43            & 0.68    & 0.71            & 1800  \\
			& Switches & 15.52       & 15.02       &  15.02       & 15.08       & 14.93      & 14.50       & 12.10       & 12.01      & \textbf{9.65}       & 9.01     \\
			\cmidrule{1-12}

			\multirow{4}[0]{*}{$20 \times 5$} 
			& Makespan & 359.06 & 373.83  & 361.26  & 373.95  & 373.54  & 342.69  & 300.70 &327.17  & \textbf{296.88} & 279.45 \\
			& Gap      & 28.5\% & 33.5\% & 29.3\% & 33.8\% & 33.7\% & 22.6\% & 7.6\% & 17.1\% & \textbf{6.2\%} & 0\%   \\
			& Time (s) & 0.32    & 0.32    & 0.32    & 0.32    & 0.32    & 0.78    & 0.84            & 1.30    & 1.41            & 1800  \\
			& Switches & 32.21       & 32.86       & 33.01       & 33.18       & 33.50       & 32.40       & 21.61       & 27.66      & \textbf{19.19}       & 20.68     \\
			\cmidrule{1-12}

			\multirow{4}[0]{*}{$15 \times 10$} 
			& Makespan & 335.05 & 306.45  & 327.73  & 298.91  & 352.88  & 326.25  & 279.47 & 294.91  & \textbf{259.34} & 239.79 \\
			& Gap      & 39.7\% & 27.8\% & 36.7\% & 23.8\% & 47.2\% & 36.1\% & 16.5\% & 23.0\% & \textbf{8.2\%} & 0\%   \\
			& Time (s) & 0.51    & 0.51    & 0.50    & 0.50    & 0.50    & 1.17   & 1.33           & 1.91    & 2.02            & 1800  \\
			& Switches & 24.46       & 24.07       & 24.24      & 24.21       & 23.83       & 23.62      & 16.03       & 20.76       & \textbf{13.79}       & 13.90     \\
			\cmidrule{1-12}

			\multirow{4}[1]{*}{$20 \times 10$} 
			& Makespan & 413.55  & 393.96  & 420.79  & 388.03  & 452.13  & 411.05 & 342.13 & 385.22  & \textbf{324.63} & 297.75 \\
			& Gap      & 38.9\% & 32.3\% & 41.3\% & 30.3\% & 51.8\% & 38.1\%  & 14.9\% & 29.4\%  & \textbf{9.0\%} & 0\%   \\
			& Time (s) & 0.71    & 0.71    & 0.71    & 0.71    & 0.71    & 1.68   & 1.76            & 3.02    & 3.20            & 1800  \\
			& Switches & 33.66      & 33.14       & 33.53      & 33.34       & 33.90       & 33.17       & 19.89       & 29.07       & \textbf{17.26}       & 18.99    \\
			\cmidrule{1-12}

			\multirow{4}[1]{*}{$30 \times 10$} 
			& Makespan & 595.15  & 566.64  & 593.82  & 554.79  & 624.53  & 579.29  & 452.11 & 547.34  & \textbf{444.70} & 410.74 \\
			& Gap      & 44.9\% & 38.0\% & 44.6\% & 35.1\% & 52.0\% & 41.0\%  & 10.1\% & 33.3\%  & \textbf{8.3\%} & 0\%   \\
			& Time (s) & 1.25    & 1.25    & 1.25    & 1.25    & 1.25    & 2.26    & 2.64            & 6.82    & 7.19           & 1800  \\
			& Switches & 51.98     & 51.05      & 52.26      & 51.73     & 51.13     & 50.57      & 26.31       & 45.23      & \textbf{25.13}       & 25.93     \\
			\cmidrule{1-12}

			\multirow{4}[1]{*}{$40 \times 10$} 
			& Makespan & 757.67  & 741.12  & 762.47 & 723.96  & 794.56  & 742.75  & 567.47 & 715.23  & \textbf{564.89} & 518.18 \\
			& Gap      & 46.2\% & 43.0\% & 47.1\% & 39.7\% & 53.3\% & 43.3\%  & 9.5\% & 38.0\%  & \textbf{9.0\%} & 0\%   \\
			& Time (s) & 2.10    & 2.10    & 2.10    & 2.10    & 2.10    & 3.21    & 3.47           & 13.18    &   14.05         & 1800  \\
			& Switches & 70.12      & 70.02      & 68.89      & 69.56      & 68.33     & 67.66      & 33.76      & 62.73      & \textbf{31.47}      & 41.82    \\
			\cmidrule{1-12}
		\end{tabular}
	\end{threeparttable}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result_2.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{Evaluation on the Synthetic datasets.}
% \renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\textbf{Size} & \textbf{Metrics} & \textbf{OR-Tools} & \textbf{FIFO\_EET} & \textbf{MWR\_EET} & \textbf{SPT\_SPT} & \textbf{RL-HGNN} & \textbf{Ours} \\
\hline
\multirow{4}{*}{10$\times$5} 
& Makespan &  &  &  &  &  &  \\
& Gap$^\dag$ & - &  &  &  &  & \\
& Time (s) & &  &  &  &  &  \\
& Pallet Switches & - & - & - &  &  & \\
\hline
\multirow{4}{*}{20$\times$5} 
& Makespan &  &  &  &  &  &  \\
& Gap$^\dag$ &  &  &  &  &  & \\
& Time (s) &  &  &  &  &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{15$\times$10} 
& Makespan &  &  &  &  &  &  \\
& Gap$^\dag$ & - &  &  &  &  &  \\
& Time (s) &  &  &  &  &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{20$\times$10} 
& Makespan & - & - & - & - &  &  \\
& Gap$^\dag$ & - & - & - & - &  &  \\
& Time (s) & - & - & - & - &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{30$\times$10} 
& Makespan & - & - & - & - & - & - \\
& Gap$^\dag$ & - & - & - & - &  &  \\
& Time (s) & - & - & - & - &  &  \\
& Pallet Switches & - & - & - &  &  &  \\
\hline
\multirow{4}{*}{40$\times$10} 
& Makespan & - & - & - & - & - & - \\
& Gap$^\dag$ & - & - & - & - & - & - \\
& Time (s) & - & - & - & - & - & - \\
& Pallet Switches & - & - & - & - & - & - \\
\hline
\end{tabular}
\begin{flushleft}
\footnotesize $^*$ The value in parentheses is the time for a single epoch. We ran multiple times and selected the best Makespan. \\
\footnotesize $^\dag$ Gap is relative to OR-Tools. Pallet Switches denotes the number of times pallets are replaced during sorting.
\end{flushleft}
\label{tab:main-results}
\end{table*}


==> AnonymousSubmission/LaTeX/Table/Table_synthetic_result_3.tex <==
\begin{table}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{Evaluation on the Synthetic datasets.}
% \renewcommand{\arraystretch}{1.3}
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Size} & \textbf{Metrics} & \textbf{OR-Tools} & \textbf{Best PDRs} & \textbf{RL-HGNN} & \textbf{Ours} \\
\hline
\multirow{4}{*}{10$\times$5} 
& Makespan &  &  &    &  \\
& Gap$^\dag$ & - &    &  & \\
& Time (s) & &  &    &  \\
& Pallet Switches & - & -   &  & \\
\hline
\multirow{4}{*}{20$\times$5} 
& Makespan &  &  &   &  \\
& Gap$^\dag$ &  &    &  & \\
& Time (s) &  &  &    &  \\
& Pallet Switches & - & -  &  &  \\
\hline
\multirow{4}{*}{15$\times$10} 
& Makespan &  &   &  &  \\
& Gap$^\dag$ & -   &  &  &  \\
& Time (s) &  &    &  &  \\
& Pallet Switches & - & -   &  &  \\
\hline
\multirow{4}{*}{20$\times$10} 
& Makespan & - &  - &  &  \\
& Gap$^\dag$ & - & - &  &  \\
& Time (s) & - & - &  &  \\
& Pallet Switches & - & - &  &  \\
\hline
\multirow{4}{*}{30$\times$10} 
& Makespan & - & -  & - & - \\
& Gap$^\dag$ & - & - &  &  \\
& Time (s) & - & -  &  &  \\
& Pallet Switches & -  &  &  &  \\
\hline
\multirow{4}{*}{40$\times$10} 
& Makespan & - & - & -  & - \\
& Gap$^\dag$ & - & - & -  & - \\
& Time (s) & - & - & -  & - \\
& Pallet Switches & - & -  & - & - \\
\hline
\end{tabular}
\begin{flushleft}
\footnotesize $^*$ The value in parentheses is the time for a single epoch. We ran multiple times and selected the best Makespan. \\
\footnotesize $^\dag$ Gap is relative to OR-Tools. Pallet Switches denotes the number of times pallets are replaced during sorting.
\end{flushleft}
\label{tab:main-results}
\end{table}


==> AnonymousSubmission/LaTeX/Table/state_graph.tex <==
\begin{table}[t]
\centering
\caption{Node, Edge and State Definitions in Dynamic Heterogeneous Graph}
\scriptsize
\setlength{\tabcolsep}{0.7em}
% \renewcommand{\arraystretch}{0.9}  % Reduce row height
% \setlength{\tabcolsep}{2.5pt} % 缩小列间距
\begin{tabular}{lll}
\toprule
\textbf{Type} & \textbf{Symbol} & \textbf{Definition}  \\

\midrule

\multirow{3}[1]{*}{Node} & Operations \((O)\) & \(O_{ij}\): The \(j\)-th operation of job \(i\) \\ 
 & Machines \((M)\) & \(M_{k}\): The \(k\)-th machine used for processing operations  \\
  & Buffer \((B)\) & \(B\): A set of buffer zones (pallets) for operation   \\
\midrule

\multirow{3}[1]{*}{Edge} & \(O\xrightarrow{}O\) & Directed edge indicating \(O_{ij}\) as the predecessor of \(O_{ij'}\) \\ 
 & \(O\leftrightarrow{}M\) & Undirected edge between \(O_{ij}\) and \(M_{k}\) when \(M_{k}\) can process \(O_{ij}\)  \\
  & \(O\leftrightarrow{}B\)  & Undirected edge between \(O_{ij}\) and \(B\) when \(O_{ij}\) has buffer constraint \\


\midrule

\multirow{3}[1]{*}{State} & \(h_{O_{ij}}\in \mathbb{R}^{18} (\forall{O_{ij}}\in O_{u(t)} )\) & Operation feature \\ 
& \(h_{M_{k}}\in \mathbb{R}^{3} (\forall{M_{k}}\in M_{u(t)} )\) & Machine feature \\ 
& \(h_{(O_{ij},M_{k})}\in \mathbb{R} (\forall{O_{ij}}\in O_{u(t)} )\) & Operation-Machine pair feature \\ 
\bottomrule
\end{tabular}

\vspace{1ex}

\label{tab:state_graph}
\end{table}

==> AnonymousSubmission/LaTeX/Table/state_graph_table.tex <==
\begin{table}[t]
\centering
\caption{Node, Edge and State Definitions in Heterogeneous Graph}
\scriptsize
\setlength{\tabcolsep}{0.32em}
% \renewcommand{\arraystretch}{0.9}  % Reduce row height
% \setlength{\tabcolsep}{2.5pt} % 缩小列间距
\begin{tabular}{lll}

\toprule
\textbf{Type} & \textbf{Symbol} & \textbf{Definition}  \\

\midrule

\multirow{3}[1]{*}{Node} & Operations \((O)\) & \(O_{ij}\): The \(j\)-th operation of job \(i\) \\ 
 & Machines \((M)\) & \(M_{k}\): The \(k\)-th machine used for processing operations  \\
  & Buffer \((B)\) & \(B\): A set of buffer zones (pallets) for operation   \\
\midrule

\multirow{3}[1]{*}{Edge} & \(O\xrightarrow{}O\) & Directed edge: \(O_{ij}\) is the predecessor of \(O_{ij'}\) \\ 
 & \(O\leftrightarrow{}M\) & Undirected edge between \(O_{ij}\) and \(M_{k}\)\\
  & \(O\leftrightarrow{}B\)  & Undirected edge between \(O_{ij}\) and \(B\) \\


\midrule

\multirow{4}[1]{*}{State} & \(h_{O_{ij}}\in \mathbb{R}^{6+T+2}\) & Operation feature \\ 
& \(h_{M_{k}}\in \mathbb{R}^{3}\) & Machine feature \\ 
& \(h_{(O_{ij},M_{k})}\in \mathbb{R}\) & Operation-Machine pair feature  \\ 
& \(B\in \mathbb{R}^{T+2}\) & Buffer feature \\ 
\bottomrule
\end{tabular}

\vspace{1ex}
\label{tab:state_graph_table}
\end{table}
